Whispering Secrets in a Crowd: Leveraging Non-Covert Users for Covert Communications

This paper establishes the fundamental limits of a multi-access system where multiple users communicate to a legitimate receiver in presence of an external warden. Only a specific subset of the users, called covert users, needs their communication to remain undetected to the warden, while the remaining non-covert users have no such constraint. The fundamental limits show a tradeoff between the different rates that are simultaneously achievable at the various users in function of the secret-key rates that the different users share with the legitimate receiver. Interestingly, the presence of the non-covert users can enhance the capacities of the covert users, especially under stringent secret-key budgets. Our findings underscore the essential requirement of employing a multiplexing (coded time-sharing) strategy to exhaust the fundamental region of all rates that are simultaneously achievable at the covert and the non-covert users. As a side-product of our results, we also establish the covert-capacity secret-key tradeoff for standard single-user and multi-access covert communication systems (without non-covert users), i.e., the largest covert rates that are achievable under given secret-key rate budgets. Previous works had only established the minimum secret-key rates required at largest covert rates.

==> plots/only_two_coverts_different_sk_budgets.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{figure}[!h]
    \centering
        
    \begin{tikzpicture}
    
        \begin{axis}[%
            width=2.919in,
            height=1.472in,
            at={(0in,0in)},
            scale only axis,
            xmin=0,
            xmax=1.5,
            xlabel style={font=\color{white!15!black}},
            xlabel={Covert rate $r_1$},
            ymin=0,
            ymax=0.9,
            xtick={0, 0.5, 1, 1.5},
            ytick={0, 0.1, 0.3, 0.6, 0.9},
            ylabel style={font=\color{white!15!black}},
            ylabel={Covert rate $r_2$},
            axis background/.style={fill=white},
            title style={font=\bfseries},
            axis x line*=bottom,
            axis y line*=left,
            legend style={legend cell align=left, align=left, draw=white!15!black}
        ]
            \addplot [color=blue, dashed]
            table[row sep=crcr]{%
                0.590040085142045	0\\
                0.727322524683288	0\\
                0.86421646684473	0\\
                0.915008283448205	0\\
                0.989376378882453	0\\
                0.989376402329208	0\\
                0.989376412588227	0\\
                0.989376413102613	0\\
                0.989376418149378	0\\
                0.989376418688559	0\\
                0.989376420096471	0\\
                0.989376420150055	0\\
                0.989376420451072	0\\
                0.989376420725411	0\\
                0.989376420793806	0\\
                0.989376421000529	0\\
                0.989376421060415	0\\
                0.989376421099576	0\\
                0.989376421102038	0\\
                0.989376421106693	0\\
                0.989376421111467	0\\
                0.989376421120797	0\\
                0.989376421127473	0\\
                0.989376421128942	0\\
                0.989376421136803	0\\
                0.989376421141755	0\\
                0.989376421143225	0\\
                0.989376421160546	0\\
                0.989376421164363	0\\
                0.989376421165387	0\\
                0.989376421176977	0\\
                0.989376421181814	0\\
                0.989376421184097	0\\
                0.989376421184191	0\\
                0.989376421187975	0\\
                0.989376421188563	0\\
                0.98937642118884	0\\
                0.989376421189369	0\\
                0.989376421189672	0\\
                0.989376421189742	0\\
                0.989376421190156	0\\
                0.989376421190182	0\\
                0.98937642119051	0\\
                0.989376421190916	0\\
                0.989376421191098	0\\
                0.989376421191354	0\\
                0.989376421191373	0\\
                0.989376421191478	0\\
                0.989376421191482	0\\
                0.98937642119153	0\\
                0.989376421191559	0\\
                0.98937642119156	0\\
                0.989376421191623	0\\
                0.989376421191632	0\\
                0.989376421191684	0\\
                0.989376421191687	0\\
                0.989376421191688	0\\
                0.989376421191692	0\\
                0.989376421191695	0\\
                0.9893764211917	0\\
                0.989376421191702	0\\
                0.989376421191703	0\\
                0.989376421191704	0\\
                0.989376421191704	0\\
                0.989376421191704	0\\
                0.989376421191704	0\\
                0.989376421191705	0\\
                0.989376421191706	0\\
                0.989376421191706	0\\
                0.989376421191706	0\\
                0.989376421191706	0\\
                0.989376421191706	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.17930956356792\\
                0	0.161235670677945\\
                0	0.00664394161950638\\
                0	0.00165704840900696\\
                0	0\\
                0.00494547695651619	0\\
                0.0211247603275154	0\\
                0.150775759962708	0\\
                0.372638769657668	0\\
                0.494885561086557	0\\
                0.548493026968616	0\\
                0.590040085142045	0\\
                };
                \addlegendentry{$k_1 \leq = 0.3 ; k_2 \leq 0.1$}
        
            \addplot [color=black, dashdotted]
            table[row sep=crcr]{%
                0	0.53792869070373\\
                0	0.537928690703655\\
                0	0.537928690703603\\
                0	0.537928690703579\\
                0	0.537928690703565\\
                0	0.537928690703562\\
                0	0.537928690703548\\
                0	0.537928690703416\\
                0	0.53792869070336\\
                0	0.537928690703105\\
                0	0.537928690702892\\
                0	0.537928690702857\\
                0	0.537928690702779\\
                0	0.537928690702762\\
                0	0.537928690702469\\
                0	0.537928690702229\\
                0	0.53792869070218\\
                0	0.537928690701465\\
                0	0.537928690701084\\
                0	0.537928690700531\\
                0	0.537928690700238\\
                0	0.53792869069976\\
                0	0.537928690697874\\
                0	0.537928690689472\\
                0	0.537928690673409\\
                0	0.537928690672045\\
                0	0.537928690642316\\
                0	0.537928690575928\\
                0	0.537928689999397\\
                0	0.537928688403223\\
                0	0.53792868575083\\
                0	0.330288382457768\\
                0	0.0952209019650919\\
                0	0.0560367842887806\\
                0	0.017317603715273\\
                0	0\\
                0.0859470071523244	0\\
                0.329792140393059	0\\
                0.329792140396689	0\\
                0.329792140397022	0\\
                0.32979214039719	0\\
                0.329792140397193	0\\
                0.329792140397226	0\\
                0.329792140397231	0\\
                0.329792140397235	0\\
                0.329792140397235	0\\
                0.329792140397235	0\\
                0.329792140397235	0\\
                0.329792140397235	0.53792869070376\\
                0.329792140397235	0.53792869070376\\
                0	0.537928690703761\\
                0	0.53792869070376\\
                0	0.53792869070376\\
                0	0.53792869070376\\
                0	0.53792869070376\\
                0	0.53792869070376\\
                0	0.537928690703759\\
                0	0.537928690703759\\
                0	0.537928690703758\\
                0	0.537928690703758\\
                0	0.537928690703757\\
                0	0.537928690703757\\
                0	0.537928690703756\\
                0	0.537928690703754\\
                0	0.537928690703752\\
                0	0.537928690703749\\
                0	0.537928690703748\\
                0	0.537928690703745\\
                0	0.537928690703742\\
                0	0.53792869070373\\
                };
                \addlegendentry{$k_1 \leq = 0.1 ; k_2 \leq 0.3$}
        
            \addplot [color=red, solid]
            table[row sep=crcr]{%
                0.00365181143660908	0.80943924492999\\
                0	0.80943924492999\\
                0	0\\
                1.47279845375481	0\\
                1.47279845375481	0.00146592982502079\\
                1.4727984537548	0.00419888683703154\\
                1.47058049329086	0.0486316781419224\\
                1.47006188127543	0.0535448958647902\\
                1.46933778771508	0.0596784937224147\\
                1.46828368056771	0.0675493295320197\\
                1.46666453939024	0.0780119601537849\\
                1.463991316905	0.0925945057412416\\
                1.46399128425755	0.092594668978392\\
                1.46194957433575	0.10226628794\\
                1.45911008028378	0.114293093273739\\
                1.45911004398648	0.114293238462872\\
                1.45499905288775	0.129642424987181\\
                1.45321246524664	0.135743065218679\\
                1.44873495919741	0.149883782973522\\
                1.44873472980488	0.149884471152692\\
                1.448734728866	0.149884473969342\\
                1.44254561146956	0.167361890349879\\
                1.43852662644877	0.17773394293052\\
                1.43852642131823	0.177734455756028\\
                1.43366262103341	0.189475361822023\\
                1.43083859224421	0.195945085651998\\
                1.4202984969379	0.218270261950649\\
                1.4202984891399	0.218270277546646\\
                1.4202984835247	0.218270288777064\\
                1.42029847686315	0.21827030210016\\
                1.40879517611537	0.240070786142964\\
                1.4053423986246	0.246198358211611\\
                1.39895129432392	0.257110622171143\\
                1.39895084016746	0.257111379098045\\
                1.39317994510565	0.266533634983951\\
                1.3832119487618	0.281969758288692\\
                1.38321191289752	0.2819698120851\\
                1.37494234486761	0.294072523905996\\
                1.37132222684718	0.29919195315081\\
                1.36208615195677	0.311808132757597\\
                1.36208610044606	0.311808201438546\\
                1.35472848176918	0.321440474383135\\
                1.34874043936157	0.32903119590319\\
                1.3487401629662	0.329031541397636\\
                1.33959901111641	0.340225578459739\\
                1.33296090063076	0.348079397370579\\
                1.32792708227438	0.353891755856519\\
                1.32398089758569	0.358366222816076\\
                1.32080527664818	0.361916633115944\\
                1.29157415974318	0.392704648712077\\
                1.29157357973071	0.392705228725986\\
                1.29157319338538	0.392705615071653\\
                1.29157313829313	0.392705670163913\\
                1.29157313385313	0.392705674603915\\
                1.29157311492407	0.39270569353297\\
                1.29157309858581	0.392705709871236\\
                1.29157303514648	0.392705773310548\\
                1.25805628037149	0.424480733484866\\
                1.25381368294345	0.428275394981122\\
                1.24834621994055	0.433097179194094\\
                1.24103663201948	0.439427326217229\\
                1.23077335600321	0.448101030097954\\
                1.2153345974992	0.460705739855744\\
                1.21533459052354	0.46070574543627\\
                1.20429147487775	0.469416374680941\\
                1.18956980958288	0.480659645250525\\
                1.18956980235586	0.480659650670789\\
                1.16900892302969	0.49570743121554\\
                1.16022874294119	0.50191587876001\\
                1.13839906937749	0.51682744090014\\
                1.13839904870726	0.516827454680288\\
                1.10822282100988	0.536304517961638\\
                1.08841751859013	0.548432468655375\\
                1.08841750629628	0.548432476031687\\
                1.06407225823847	0.562687326422125\\
                1.04970512631986	0.57078226820624\\
                0.994227148512654	0.600023462114565\\
                0.994225478793921	0.600024296975211\\
                0.994225451060663	0.600024310841839\\
                0.99422511396352	0.600024479390346\\
                0.929712466302601	0.630443998322922\\
                0.909442296809684	0.639290954276899\\
                0.870741507627169	0.655317221133943\\
                0.870741353990206	0.655317282588734\\
                0.834433943509701	0.669381531444265\\
                0.768572671352729	0.692683652859584\\
                0.768572662858532	0.692683655690983\\
                0.768572651765313	0.692683659388722\\
                0.710853934666555	0.710948583339046\\
                0.684711411615876	0.718603599806975\\
                0.615620848631157	0.737094130473709\\
                0.61562084567856	0.737094131211858\\
                0.558214611016242	0.750641015444335\\
                0.510028963311393	0.760809881887361\\
                0.510027782519494	0.760810118045403\\
                0.434152431038271	0.774708931258246\\
                0.377488804848193	0.783474419597806\\
                0.333765802418392	0.789328684219899\\
                0.299095985223832	0.793421009213859\\
                0.270978734610741	0.79638863941382\\
                0.00760628809172871	0.80943924492999\\
                0.00365181143660908	0.80943924492999\\
                };
                \addlegendentry{$k_1 \leq = 0.6 ; k_2 \leq 0.6$}

        \end{axis}
    \end{tikzpicture}%
    \caption{Rate-region $(r_1,r_2)$ at different secret-key rates budgets $k_1,k_2$.}
    
    \label{fig:only_two_coverts}
\end{figure}
